Alethe: Towards a Generic SMT Proof Format (extended abstract)

The first iteration of the proof format used by the SMT solver veriT was presented ten years ago at the first PxTP workshop. Since then the format has matured. veriT proofs are used within multiple applications, and other solvers generate proofs in the same format. We would now like to gather feedback from the community to guide future developments. Towards this, we review the history of the format, present our pragmatic approach to develop the format, and also discuss problems that might arise when other solvers use the format.

==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{Chantal Keller and Mathias Fleury (Eds.): Seventh Workshop\\
on Proof eXchange for Theorem Proving (PxTP)\\
EPTCS 336, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.336.6}{10.4204/EPTCS.336.6}}
\pdfoutput=1

